Taxonomy-Aware Continual Semantic Segmentation in Hyperbolic Spaces for Open-World Perception

Semantic segmentation models are typically trained on a fixed set of classes, limiting their applicability in open-world scenarios. Class-incremental semantic segmentation aims to update models with emerging new classes while preventing catastrophic forgetting of previously learned ones. However, existing methods impose strict rigidity on old classes, reducing their effectiveness in learning new incremental classes. In this work, we propose Taxonomy-Oriented Poincar\'e-regularized Incremental-Class Segmentation (TOPICS) that learns feature embeddings in hyperbolic space following explicit taxonomy-tree structures. This supervision provides plasticity for old classes, updating ancestors based on new classes while integrating new classes at fitting positions. Additionally, we maintain implicit class relational constraints on the geometric basis of the Poincar\'e ball. This ensures that the latent space can continuously adapt to new constraints while maintaining a robust structure to combat catastrophic forgetting. We also establish eight realistic incremental learning protocols for autonomous driving scenarios, where novel classes can originate from known classes or the background. Extensive evaluations of TOPICS on the Cityscapes and Mapillary Vistas 2.0 benchmarks demonstrate that it achieves state-of-the-art performance. We make the code and trained models publicly available at http://topics.cs.uni-freiburg.de.

==> images/graphs/miou_over_time_rebuttal.tex <==
\begin{figure} 
        \centering
        \resizebox{0.75\columnwidth}{!}{%
        \begin{tikzpicture} [font=\small]
        \begin{axis}[
            title={},
            ylabel={mIoU [\%]},
            legend style={font=\footnotesize},
            xlabel={Incremental step},
            xmin=0.5, xmax=10.5,
            ymin=28, ymax=93,
            ytick={30,40,50, 60, 70, 80},
            xtick={1,3,5,7,9,10},
            legend pos=north east,
            legend columns=3, 
            ymajorgrids=true,
            grid style=dashed,
            height=6cm
        ]

        \addplot[
            color=color_red,
            mark=square,
            line width=0.4mm,
            ]
            coordinates {
            (1,66.46)(2,68.28)(3,68.63)(4,67.38)(5,68.97)(6,67.24)(7,65.66)(8,60.24)(9,59.55)(10,59.36)
            };
        \addlegendentry{\net}
        \addplot[
            color=color_red,
            mark=x,
            line width=0.4mm,
            ]
            coordinates {
            (1,60.94)(2,63.56)(3,64.78)(4,63.41)(5,65.27)(6,64.21)(7,61.38)(8,56.71)(9,55.97)(10,55.83)
            };
        \addlegendentry{\net$_{b30}$}
        \addplot[
            color=color_brown,
            mark=triangle,
            line width=0.4mm,
            ]
            coordinates {
            (1,62.59)(2,64.98)(3,64.45)(4,59.35)(5,60.83)(6,58.26)(7,54.51)(8,49.93)(9,46.17)(10,45.73)
            };
        \addlegendentry{MiB\cite{cermelli2020mib}}
                \addplot[
            color=color_green,
            mark=star,
            line width=0.4mm,
            ]
            coordinates {
            (1,62.59)(2,64.95)(3,64.59)(4,60.11)(5,61.34)(6,58.23)(7,55.93)(8,50.23)(9,48.36)(10,46.55)
            };
        \addlegendentry{MiB+AWT~\cite{goswami2023attribution}}
        \addplot[
            color=color_purple,
            mark=o,
            line width=0.4mm,
            ]
            coordinates {
            (1,58.57)(2,61.44)(3,61.2)(4,56.63)(5,56.92)(6,55.31)(7,51.87)(8,48.01)(9,45.13)(10,42.96)
            };
        \addlegendentry{PLOP~\cite{Douillard2020PLOPLW}}
                 \addplot[
            color=color_orange,
            mark=diamond,
            line width=0.4mm,
            ]
            coordinates {
            (1,63.76)(2,65.55)(3,65.93)(4,61.30)(5,62.55)(6,60.32)(7,56.47)(8,51.84)(9,50.30)(10,48.92)
            };
        \addlegendentry{DKD~\cite{baek2022_dkd}}
        \addplot[
            color=color_blue,
            mark=x,
            line width=0.4mm,
            ]
            coordinates {
            (1,48.04)(2,46.27)(3,46.21)(4,41.77)(5,44.27)(6,41.94)(7,40.78)(8,39.06)(9,34.47)(10,32.78)
            };
        \addlegendentry{Microseg~\cite{zhang22_microseg}}
    \end{axis}
    \end{tikzpicture}}
\caption{Performance at every increment on Cityscapes 10-1 (10 task) setting.}
\label{fig:miou10tasks_rebut}
\end{figure}

==> sections/old.tex <==
% \begin{table*}[h]
% \caption{Continual Semantic Segmentation results on ADE20k in Mean IoU (\%)}
% \label{table_ade20k}
% \begin{center}
% \begin{tabular}
% {l|cccc||cccc||cccc}
%  \toprule
%  & \multicolumn{4}{c}{\textbf{100-50 (2 tasks)}} & \multicolumn{4}{c}{\textbf{50-50 (3 tasks)}} & \multicolumn{4}{c}{\textbf{100-10 (6 tasks)}}\\
% \textbf{Method} & 0-100 & 101-150 & all & avg & 0-50 & 51-150 & all & avg & 0-100 & 101-150 & all & avg \\
% \midrule
% LwF & & & & & & & & & & & &\\
% MiB & & & & & & & & & & & &\\
% EWC & & & & & & & & & & & &\\
% PLOP & & & & & & & & & & & &\\
% UCD & & & & & & & & & & & &\\
% Ours & & & & & & & & & & & &\\
% \hline
% \end{tabular}
% \end{center}
% \end{table*}

% \begin{table*}[h]
% \caption{Continual Semantic Segmentation results on PascalVOC in Mean IoU (\%)}
% \label{table_ade20k}
% \begin{center}
% \begin{tabular}
% {l|ccc||ccc||ccc}
%  \toprule
%  & \multicolumn{3}{c}{\textbf{19-1 (2 tasks)}} & \multicolumn{3}{c}{\textbf{15-5 (2 tasks)}} & \multicolumn{3}{c}{\textbf{15-1 (6 tasks)}}\\
% \textbf{Method} & 0-19 & 20 & all & 0-15 & 15-20 & all & 0-15 & 16-20 & all \\
% \midrule
% LwF & & & & & & & & & \\
% MiB & & & & & & & & & \\
% EWC & & & & & & & & & \\
% PLOP & & & & & & & & & \\
% UCD & & & & & & & & & \\
% Ours & & & & & & & & & \\
% \hline
% \end{tabular}
% \end{center}
% \end{table*}





%    \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%        magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%    \end{figure}
   

% Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity ÒMagnetizationÓ, or ÒMagnetization, MÓ, not just ÒMÓ. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write ÒMagnetization (A/m)Ó or ÒMagnetization {A[m(1)]}Ó, not just ÒA/mÓ. Do not label axes with a ratio of quantities and units. For example, write ÒTemperature (K)Ó, not ÒTemperature/K.Ó




\begin{table*}[h]
\caption{Continual Hierarchical Semantic Segmentation results on Cityscapes in Mean IoU (\%)}
\label{table_city2}
\begin{center}
\begin{tabular}
{l|ccc||ccc}
 \toprule
 & \multicolumn{3}{c}{\textbf{h:7-4 (4 tasks)}} & \multicolumn{3}{c}{\textbf{h:7-18 (2 tasks)}}\\
\textbf{Method} & 0-7 & 8-25 & all & 0-7 & 8-25 & all\\
\midrule
PLOP~\cite{Douillard2020PLOPLW} & 88.56 & 18.14 & 20.75 & 88.73 & 15.06 & 17.99 \\
MiB~\cite{cermelli2020mib} & 77.66 & 6.61 & 9.83 & 90.10 & 5.71 & 9.64 \\
MiB + AWT~\cite{goswami2023attribution} & 84.65 & 10.46 & 13.64 & 90.19 & 5.61 & 9.56 \\
DKD~\cite{baek2022_dkd} & 89.46 & 0.56 & 4.98 & 89.19 & 4.29 & 8.32 \\
MicroSeg~\cite{zhang22_microseg} & 86.39 & 1.63 & 5.79 & 86.37 & 7.71 & 11.26 \\
% urs (Hier) & 89.24 & 30.76 & 32.14 & & \\
\net~(Ours) & \textcolor{gray}{87.27} & \textcolor{gray}{36.17} & \textcolor{gray}{36.92} & \textcolor{gray}{89.89} & \textcolor{gray}{15.29} & \textcolor{gray}{18.25} \\
\hline
\end{tabular}
\end{center}
\end{table*}


\begin{table*}[h]
\caption{Continual Hierarchical Semantic Segmentation results on Mapillary Vistas v2 in Mean IoU (\%)}
\label{table_map}
\begin{center}
\begin{tabular}{l|ccc||ccc}
 \toprule
 & \multicolumn{3}{c}{\textbf{40-21 (5 tasks)}} & \multicolumn{3}{c}{\textbf{40-83 (2 tasks)}} \\
\textbf{Method} & 0-40 & 41-124 & all & 0-40 & 41-112 & all \\
\midrule
PLOP~\cite{Douillard2020PLOPLW} & 17.79 & 3.14 & 6.64 & 19.15 & 5.52 & 9.51 \\
MiB~\cite{cermelli2020mib} & 16.49 & 6.51 & 8.86 & 19.38 & 13.61 & 11.64 \\
MiB + AWT~\cite{goswami2023attribution} & 17.75 & 11.16 & 12.84 & 19.76 & 13.47 & 15.47 \\
DKD~\cite{baek2022_dkd} & 28.04 & 1.53 & 8.06 & 24.24 & 3.20 & 9.15 \\
\net~(Ours) & & & & &  \\
\hline
\end{tabular}
\end{center}
\end{table*}

\begin{table}
\centering
\caption{Continual semantic segmentation results on Cityscapes in mIoU (\%).}
\label{tab:ab_elem}
\begin{tabular}
{l|lll|ccc}
 \toprule
 & \multicolumn{6}{c}{\textbf{15-1 (6 tasks)}}\\
\textbf{Space} & \textbf{Softmax} & \textbf{Sigmoid} &\textbf{Hier.}  & 1-14 & 15-19 & all \\
\midrule
\multirow{3}{*}{Euclidean} & \checkmark & & & \textcolor{gray}{66.56} & \textcolor{gray}{19.68} & \textcolor{gray}{51.51} \\
& & \checkmark &  & \textcolor{gray}{62.17} & \textcolor{gray}{21.10} & \textcolor{gray}{54.61} \\
& \checkmark & & \checkmark & \textcolor{gray}{72.79} & \textcolor{gray}{32.35} & \textcolor{gray}{59.04} \\
& & \checkmark & \checkmark & \textcolor{gray}{62.17} & \textcolor{gray}{21.10} & \textcolor{gray}{48.80} \\
\midrule
% \multirow{3}{*}{Hyperbolic} & \checkmark & & & 68.46 & 24.01 & 53.92 \\
\multirow{3}{*}{Hyperbolic} & \checkmark & & & 72.72 & 37.13 & 60.19\\
& \checkmark & & \checkmark & 72.79 & 32.35 & 59.04 \\
& & \checkmark & & 71.65 & 37.09 & 59.43 \\
& & \checkmark & \checkmark & 73.04 & 39.74 & 61.06 \\
% & \checkmark & \checkmark & \checkmark & 68.42 & 23.75 & 53.83 \\
\hline
\end{tabular}
\end{table}

\begin{table*}
\centering
\caption{Continual semantic segmentation results on Mapillary Vistas~2.0 in mIoU (\%). Tasks defined as $\mathcal{C}^1$-$\mathcal{C}^T$($T$ tasks) and $h$ class hierarchy increments.}
\label{tab:map}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|p{0.7cm}p{0.8cm}p{0.7cm}|p{0.7cm}p{0.8cm}p{0.7cm}|p{0.7cm}p{0.8cm}p{0.7cm}|p{0.7cm}p{0.8cm}p{0.7cm}|p{0.7cm}p{0.8cm}p{0.7cm}}
 \toprule
 & \multicolumn{3}{c|}{\textbf{72-39 (2 tasks)}} & \multicolumn{3}{c|}{\textbf{42-30 (3 tasks)}} & \multicolumn{3}{c|}{\textbf{72-10 (5 tasks)}} & \multicolumn{3}{c|}{\textbf{39-83 (2 tasks)h}} & \multicolumn{3}{c}{\textbf{39-21 (5 tasks)h}} \\
 \cmidrule{2-16}
\textbf{Method} & 0-72 & 72-111 & all & 0-42 & 43-111 & all & 0-72 & 72-111 & all & 0-39 & 40-123 & all & 0-39 & 40-123 & all \\
\midrule
PLOP~\cite{Douillard2020PLOPLW} & 20.49 & 8.59 & 16.44 & 20.83 & 8.97 & 14.59 & 18.12 & 5.74 & 13.83 & 19.15 & 5.52 & 9.51 & 17.79 & 3.14 & 6.64 \\
MiB~\cite{cermelli2020mib} & 21.72 & 12.59 & 18.26 & 16.72 & 11.48 & 13.77 & 15.10 & 8.43 & 12.58 & 19.38 & 13.61 & 11.64 & 16.49 & 6.51 & 8.86 \\
MiB + AWT~\cite{goswami2023attribution} & 21.76 & 14.23 & 19.35 & 18.33 & 13.27 & 15.89 & 15.78 & 9.69 & 13.91 & 19.76 & 13.47 & 15.47 & 17.75 & 11.16 & 12.84 \\
DKD~\cite{baek2022_dkd} & \textbf{25.07} & 13.08 & 20.94 &  \textbf{25.49} & 12.82 & 18.74 & \textbf{22.71} & 11.03 & 18.65 & \textbf{24.24} & 3.20 & 9.15 & \textbf{28.04} & 1.53 & 8.06 \\
MicroSeg~\cite{zhang22_microseg} & 9.51 & 5.12 & 7.99 & 
9.39 & 4.19 & 6.62 & 8.38 & 3.46 & 6.65 & 12.70 & 1.07 & 4.41 & 13.69 & 0.80 & 4.08 \\ 
\midrule
\net~(Ours) & 23.81 & \textbf{18.40} & \textbf{21.81} & 23.76 &  \textbf{17.78} &  \textbf{20.35} &  22.10 & \textbf{14.55} & \textbf{19.20} & 24.16 & \textbf{21.49} & \textbf{21.94} & 26.67 & \textbf{22.57} & \textbf{23.35} \\
\hline
\end{tabular}
\vspace{-0.2cm}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}
\centering
\caption{Continual semantic segmentation results on Cityscapes in mIoU (\%). Tasks defined as $\mathcal{C}^1$-$\mathcal{C}^T$($T$ tasks) and $h$ class hierarchy increments.Relative decrease in performance on $\mathcal{C}^1$ is recorded in (\%).}
\label{tab:cityap}
\setlength{\tabcolsep}{4pt}
\begin{tabular}
{l|lcc|lcc|lcc|lcc}
 \toprule
 & \multicolumn{3}{c|}{\textbf{14-1 (6 tasks)}} & \multicolumn{3}{c|}{\textbf{10-1 (10 tasks)}} & \multicolumn{3}{c|}{\textbf{7-4 (4 tasks)h}} & \multicolumn{3}{c}{\textbf{7-18 (2 tasks)h}}\\
  \cmidrule{2-13}
\textbf{Method} & 1-14 & 15-19 & all & 1-10 & 11-19 & all & 0-7 & 8-25 & all & 0-7 & 8-25 & all\\
\midrule
PLOP~\cite{Douillard2020PLOPLW} & 63.54($\downarrow$3.64)& 15.38 & 48.33 & 60.75($\downarrow$5.43) & 27.97 & 42.96 & 88.56($\downarrow$1.25) & 18.14 & 20.75 & 88.73($\downarrow$1.07) & 15.06 & 17.99 \\
MiB~\cite{cermelli2020mib} & 66.37($\downarrow$5.75) & 14.36 & 50.05 & 61.80($\downarrow$9.8) & 32.97 & 45.73 & 77.66($\downarrow$13.0) & 6.61 & 9.83 & 90.10($\downarrow$0.0) & 5.71 & 9.64 \\
MiB + AWT~\cite{goswami2023attribution} & 65.60($\downarrow$6.84) & 19.19 & 50.72 & 60.97($\downarrow$11.07) & 35.70 & 46.55 & 84.65($\downarrow$5.16) & 10.46 & 13.64 & 90.19($\downarrow$0.0) & 5.61 & 9.56 \\
DKD~\cite{baek2022_dkd} & 68.83($\downarrow$3.21) & 14.70 & 51.86 & 66.77($\downarrow$4.51) & 34.52 & 48.92 & 89.46($\downarrow$0.0) & 0.56 & 4.98 & 89.19($\downarrow$0.1)& 4.29 & 8.32 \\
MicroSeg~\cite{zhang22_microseg} & 51.35($\downarrow$8.86) & 11.61 & 38.84 & 44.37($\downarrow$15.73) & 23.55 & 32.78 & 86.39($\downarrow$0.0) & 1.63 & 5.79 & 86.37($\downarrow$0.0) & 7.71 & 11.26 \\
\midrule
\net~(Ours) & \textbf{73.03($\downarrow$2.43)} & \textbf{42.47} & \textbf{61.74} & \textbf{71.37($\downarrow$1.99)} & \textbf{52.62} & \textbf{59.36} &
\textbf{90.02}($\downarrow$0.5) & \textbf{51.31} & \textbf{50.69} & 
\textbf{90.33}($\downarrow$0.2) & \textbf{61.62} & \textbf{59.98} \\
\hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}


\begin{table*}
\centering
\caption{Continual semantic segmentation results on Mapillary Vistas~2.0 in mIoU (\%). Tasks defined as $\mathcal{C}^1$-$\mathcal{C}^T$($T$ tasks) and $h$ class hierarchy increments. Relative decrease in performance on $\mathcal{C}^1$ is recorded in (\%).}
\label{tab:mapap}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|p{1.7cm}p{0.8cm}p{0.7cm}|p{1.7cm}p{0.8cm}p{0.7cm}|p{1.7cm}p{0.8cm}p{0.7cm}|p{1.7cm}p{0.8cm}p{0.7cm}}
 \toprule
 & \multicolumn{3}{c|}{\textbf{51-30 (3 tasks)}} & \multicolumn{3}{c|}{\textbf{71-10 (5 tasks)}} & \multicolumn{3}{c|}{\textbf{39-84 (2 tasks)h}} & \multicolumn{3}{c}{\textbf{39-21 (5 tasks)h}} \\
 \cmidrule{1-13}
\textbf{Method} & 0-42 & 43-111 & all & 0-72 & 72-111 & all & 0-39 & 40-123 & all & 0-39 & 40-123 & all \\
\midrule
PLOP~\cite{Douillard2020PLOPLW} & 20.83 \textbf{($\downarrow$17.96)} & 8.97 & 14.59 & 18.12 ($\downarrow$27.17) & 5.74 & 13.83 & 19.15 ($\downarrow$44.38)& 5.52 & 9.51 & 17.79 ($\downarrow$77.37) & 3.14 & 6.64 \\
MiB~\cite{cermelli2020mib} & 16.72 ($\downarrow$34.15) & 11.48 & 13.77 & 15.10 ($\downarrow$39.31) & 8.43 & 12.58 & 19.38 ($\downarrow$43.71) & 13.61 & 11.64 & 16.49 ($\downarrow$52.11)& 6.51 & 8.86 \\
MiB + AWT~\cite{goswami2023attribution} & 18.33 ($\downarrow$27.81) & 13.27 & 15.89 & 15.78 ($\downarrow$36.58) & 9.69 & 13.91 & 19.76 ($\downarrow$42.61)& 13.47 & 15.47 & 17.75 ($\downarrow$48.45) & 11.16 & 12.84 \\
DKD~\cite{baek2022_dkd} & \textbf{25.49} ($\downarrow$22.48)& 12.82 & 18.74 & \textbf{22.71} ($\downarrow$19.27) & 11.03 & 18.65 & \textbf{24.24} ($\downarrow$36.69)& 3.20 & 9.15 & \textbf{28.04} ($\downarrow$26.77) & 1.53 & 8.06 \\
MicroSeg~\cite{zhang22_microseg} & 9.39 ($\downarrow$28.54) & 4.19 & 6.62 & 8.38 ($\downarrow$36.71) & 3.46 & 6.65 & 12.70 ($\downarrow$42.92)& 1.07 & 4.41 & 13.69 ($\downarrow$38.47)& 0.80 & 4.08 \\ 
\midrule
\net~(Ours) & 23.76 ($\downarrow$18.88) & \textbf{17.78} &  \textbf{20.35} &
22.10 \textbf{($\downarrow$16.54)} & \textbf{14.55} & \textbf{19.20} 
& 24.16 \textbf{($\downarrow$32.94)} & \textbf{21.49} & \textbf{21.94}
& 26.67 \textbf{($\downarrow$25.98)} & \textbf{22.57} & \textbf{23.35} \\
\hline
\end{tabular}
\vspace{-0.2cm}
\end{table*}
